Partitioned Variational Inference: A Framework for Probabilistic Federated Learning

The proliferation of computing devices has brought about an opportunity to deploy machine learning models on new problem domains using previously inaccessible data. Traditional algorithms for training such models often require data to be stored on a single machine with compute performed by a single node, making them unsuitable for decentralised training on multiple devices. This deficiency has motivated the development of federated learning algorithms, which allow multiple data owners to train collaboratively and use a shared model whilst keeping local data private. However, many of these algorithms focus on obtaining point estimates of model parameters, rather than probabilistic estimates capable of capturing model uncertainty, which is essential in many applications. Variational inference (VI) has become the method of choice for fitting many modern probabilistic models. In this paper we introduce partitioned variational inference (PVI), a general framework for performing VI in the federated setting. We develop new supporting theory for PVI, demonstrating a number of properties that make it an attractive choice for practitioners; use PVI to unify a wealth of fragmented, yet related literature; and provide empirical results that showcase the effectiveness of PVI in a variety of federated settings.

==> exp.tex <==
\subsection{UCI Classification}
\label{sec:experiments:uci}
We consider three binary classification tasks available on the UCI machine learning repository \citep{dua2019uci}: \textit{adult}, with the task being to predict whether income exceeds \$50,000/year based on census data; \textit{bank}, with the task being to predict if a client will subscribe to a term deposit; and \textit{credit}, with the task being the predict whether individuals default on payments. All three tasks contain sensitive financial information, motivating the privacy constraint of federated learning. For each dataset, categorical input features are converted into multiple binary features---the increased input dimension is shown. $\eta$ indicates the proportion of positive labels within the dataset. 

For each of the federated learning schemes, we perform approximate inference of the parameters of a logistic regression model. The posterior predictive distribution $p(y_* = 1 | \xvec_*, \yvec)$ is approximated using the probit approximation \citep{spiegelhalter1990sequential}. We follow the dataset distribution scheme of \cite{sharma2019differentially} to split each dataset into $K=10$ partitions---five `small' and five `large' partitions. For each task, we consider a homogeneous split A and highly inhomogeneous split B. A detailed description of the datasets and corresponding partitions is provided in \ref{}.

\begin{figure}
    \begin{subfigure}[h]{\textwidth}
    \centering
    \includegraphics[width=.85\textwidth]{new/figs/uci/adult_pp_coms.png}
    \caption{Adult}
    \label{fig:adult_pvi}
    \end{subfigure}
    %
    \begin{subfigure}[h]{\textwidth}
    \centering
    \includegraphics[width=.85\textwidth]{new/figs/uci/bank_pp_coms.png}
    \caption{Bank}
    \label{fig:bank_pvi}
    \end{subfigure}
    %
    \begin{subfigure}[h]{\textwidth}
    \centering
    \includegraphics[width=.85\textwidth]{new/figs/uci/credit_pp_coms.png}
    \caption{Credit}
    \label{fig:credit_pvi}
    \end{subfigure}
    \label{fig:uci_pvi}
    \caption[Predictive performance on the UCI classification tasks.]{A comparison between the predictive performance of the federated learning schemes on each of the UCI classification tasks. The mean $\pm$ standard deviation averaged over five random initialisations is shown. See text for details.}
\end{figure}

\subsubsection{Empirical results agree with theory. PVI more efficient than global VI.}
Figures \ref{fig:adult_pvi}, \ref{fig:bank_pvi} and \ref{fig:credit_pvi} compare the predictive performance of the approximate posteriors learnt by each of the federated learning schemes on each of the three UCI binary classification tasks. A damping factor of $\lambda = 0.2$ is used for synchronous PVI. For both splits, we observe that both sequential and synchronous PVI converges towards the predictive performance obtained by the `optimal' approximate posterior learnt by global VI---this is in accordance with the theory presented in Section \ref{}. For the homogeneous split A, convergence is achieved after a single round of communications.\footnote{This corresponds to a single communication for synchronous PVI and $K$ communications for sequential PVI.} Convergence takes noticeably longer for the inhomogeneous split B, but is nonetheless achieved after only a few rounds of communications. Importantly, the results demonstrate that PVI is able to recover the predictive performance obtained using global VI with far greater communication efficiency. 

\subsubsection{Where and why do the other models go wrong?}
Despite being relatively simple tasks, the plots reveal the comparatively poor performance of both BCM methods and VCL relative to PVI in the presence of inhomogeneity. Although the posterior distribution is identifiable, the client-level approximate factors are interdependent and so a single round of communications---as with BCM methods---is unable to identify the globally optimal approximate posterior. Similarly, the poor performance of VCL arises due to the interdependence of approximate factors and accumulation of approximation errors, the latter resulting in an approximate posterior biased towards performing well on the distribution of the dataset visited last. This explains the relatively high variance in final test set performance of VCL. 

The inadequacies of BCM and VCL demonstrate the importance of revisiting clients to model interdependencies between approximate factors. Yet, this is not sufficient---we also need the deletion step. Without the deletion step of PVI, streaming VB `over-counts' the observations resulting in over-sharpening of the likelihood and overfitting, as illustrated by the predictive performance plot on the credit dataset.\footnote{The same degradation in predictive performance does not occur for the larger adult and bank datasets. Because the datasets are so large and the prior distribution relatively vague, the likelihood is much sharper than the prior and the posterior distribution resembles a delta on the maximum likelihood estimate. Since the maximum likelihood estimate is independent on the number of data points, both streaming VB and PVI converge towards the same solution.} 

\subsection{Mortality Prediction}
\label{sec:experiments:mp}
In this section we consider the mortality prediction task of the MIMIC-III dataset \citep{johnson2016mimic, harutyunyan2019multitask}. The dataset consists of recordings of 17 clinical variables recorded over the first 48 hours of each ICU stay, of which there are 42,276, corresponding to 33,798 unique patients. Each of the 17 recordings is divided into seven subsequences---full time series; first 10\% of time; first 25\% of time, first 50\% of time, last 50\% of time, last 25\% of time; and last 10\% of time---from which six statistical features are extracted. In total, each ICU stay is represented by a $17\times 7 \times 6 = 714$ dimensional feature vector. We reduce this to $D=50$ dimensional vectors by identifying the $50$ most important features according to the weights of a MAP trained logistic regression model.

We construct $K=5$ inhomogeneous partitions of the data by performing k-means clustering on the inputs, the purpose being to simulate the inhomogeneity of patients that one might observe at different hospitals. See \ref{} for details. We compare the performance of the federated learning methods in performing approximate inference in a logistic regression model and two-layered BNN with 100 hidden units per layer. A damping factor of $\lambda = 0.4$ is used for synchronous PVI. Figures \ref{fig:mp_pvi_lr} and \ref{fig:mp_pvi_bnn} plot the predictive performance of the methods.

\begin{figure}
    \begin{subfigure}[h]{\textwidth}
    \centering
    \includegraphics[width=\textwidth]{new/figs/mortality/mortality_logreg_pp_coms.png}
    \caption{Logistic regression model.}
    \label{fig:mp_pvi_lr}
    \end{subfigure}
    %
    \begin{subfigure}[h]{\textwidth}
    \centering
    \includegraphics[width=\textwidth]{new/figs/mortality/mortality_bnn2l_pp_coms.png}
    \caption{Two-layered BNN with 100 hidden units.}
    \label{fig:mp_pvi_bnn}
    \end{subfigure}
    \label{fig:mp_pvi}
    \caption[Predictive performance on the mortality prediction classification task using a logistic regression model.]{A comparison between the predictive performance of the federated learning schemes on the mortality prediction tasks. The mean $\pm$ standard deviation averaged over five random initialisations is shown. See text for details.}
\end{figure}

\subsubsection{Results agree with theory in both simple and complex models.}
Both PVI methods converge towards the same predictive performance achieved by global VI---doing so in far fewer communications---consolidating the observations made in Section \ref{sec:experiments:uci} and demonstrating the effectiveness of PVI in more complex models.

\subsubsection{Non-identifiability harms performance, particularly BCM.}
Convergence is noticeably smoother for the simpler logistic regression model than for the BNN, a consequence of the approximate posterior of the BNN being more complex. In particular, the non-identifiability of the approximate posterior results in poor predictive performance of BCM methods as the client-level approximate posteriors are unlikely to have converged towards the same mode, thus are unlikely to agree upon aggregation.

\subsection{Federated MNIST}
\label{sec:experiments:fmnist}
The MNIST multi-class classification task \citep{lecun1998gradient} consists of 60,000 $28\times 28$ greyscale images of handwritten digits between 0 and 9. We consider performing federated learning on two distinct partitions of the dataset: a homogeneous split, in which the dataset is partitioned equally into $K=10$ groups of 6,000 datapoints each; and the inhomogeneous split of \cite{mcmahan2017communication}, in which the dataset is partitioned into $K=100$ groups of 600 datapoints, with each group consisting of examples of just two digits. The inhomogeneous split is highly non-IID and was introduced with the intention of testing federated learning algorithms to their limits.

We investigate the performance of the federated learning methods in performing approximate inference in a single-layered BNN with 200 hidden units. For synchronous PVI a damping factor of $\lambda = 0.2$ is used for the homogeneous split and $\lambda = 0.025$ is used for the inhomogeneous split. In both cases, we found this to be the smallest damping factor necessary for stable convergence.

\subsubsection{Homogeneous Split}
Figure \ref{fig:fmnist_homo_pvi} compares the performance of federated learning schemes on the homogeneous split of the MNIST dataset.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\textwidth]{new/figs/fmnist/fmnist_homogeneous_pp_coms.png}
    \caption[Predictive performance on the homogeneous split of the MNIST classification task.]{Plots of the predictive performance of the federated learning schemes on the homogeneous split of the MNIST classification task. The split is constructed by randomly partitioning the 60,000 training images into $K=10$ partitions. The mean $\pm$ standard deviation computed using five random initialisations is shown. See text for details.}
    \label{fig:fmnist_homo_pvi}
\end{figure}

As for the simpler binary classification tasks, the predictive performance of both PVI methods converges towards the same asymptote as global VI with far greater communication efficiency. Both BCM methods perform poorly, which again owes to the non-identifiability of the approximate posterior. VCL achieves reasonable predictive performance; yet, it is evident that by revisiting clients and modifying their contribution to the approximate posterior---as in sequential PVI---predictive performance can be improved. Without the deletion step, streaming VB overfits the training dataset which results in a degradation in test set performance.

% A striking feature of the global VI performance curves is that the best predictive performance is achieved before convergence. This is an implication of the over-pruning effect described in \ref{}. The final row of Figure \ref{fig:fmnist_homo_pvi} plots the proportion of over-pruned parameters during training\footnote{A parameter, $\theta_i$, is marked as pruned if $\KL{q(\theta_i)}{p(\theta_i)} < 0.1$.}. Observe that the sudden increase in pruned parameters aligns with the worsening in predictive performance, demonstrating its detrimental effect. A frequently used technique for mitigating over-pruning is early stopping; we investigate the effects of which in Section \ref{}.

A pathology of mean-field variational approximations to BNNs is the over-pruning effect . Figure \ref{fig:fmnist_homo_pvi} demonstrates this in full effect, showing that as the number of pruned parameters increases the predictive performance worsens.\footnote{A parameter, $\theta_i$, is marked as pruned if $\textrm{KL}(q(\theta_i)\|p(\theta_i)) < 0.1$.} To mitigate this effect, we consider applying early stopping to the local free-energy optimisations by checking for convergence of the expected log-likelihood term. Rather than initialise at the context distribution, it is important to initialise the approximate posteriors at a `tight' distribution for all updates to ensure early stopping can be applied\footnote{If initialised at the context distribution as before, the local free-energies do not get the opportunity to stop early.}. Figure \ref{fig:fmnist_homo_es_pvi} compares the performance of the federated learning schemes with early stopping on the homogeneous split. 

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\textwidth]{new/figs/fmnist/fmnist_homogeneous_pp_coms_es.png}
    \caption[Predictive performance on the homogeneous split of the MNIST classification task when early stopping is applied.]{Plots of the predictive performance of the federated learning schemes on the homogeneous split of the MNIST classification task. The solid lines indicate the use of early stopping, whereas the dashed lines indicate the free-energies are optimised until convergence. The mean $\pm$ standard deviation computed using five random initialisations is shown. See text for details.}
    \label{fig:fmnist_homo_es_pvi}
\end{figure}

Observe that the use of early stopping is able to identify the best predictive performance for global VI with good precision, indicating its effectiveness. For the PVI methods, the approximate posterior increasingly overfits to the training dataset. Unlike streaming VB, however, this does not correspond to a worsening in test set predictive performance: both sequential and synchronous PVI achieve a final test set negative log-likelihood better than that achieved by global VI.

\subsubsection{Inhomogeneous Split}
Figure \ref{fig:fmnist_inhomo_pvi} compares the performance of the federated learning schemes on the inhomogeneous split of the MNIST dataset. Note that the performance metrics are plotted on the log-scale, as the variation between the performance of each method is significantly greater than in any of the previous experiments.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\textwidth]{new/figs/fmnist/fmnist_inhomogeneous_pp_coms.png}
    \caption[Predictive performance on the inhomogeneous split of the MNIST classification task.]{Plots of the predictive performance of the federated learning schemes on the inhomogeneous split of the MNIST classification task. The split is constructed by partitioning the 60,000 training images into $K=100$ partitions, each with at most two digits. The mean $\pm$ standard deviation computed using five random initialisations is shown. See text for details.}
    \label{fig:fmnist_inhomo_pvi}
\end{figure}

Despite using inhomogeneous mini-batches global VI converges towards the same predictive performance as the homogeneous case, albeit with far worse communication efficiency, reaching a test error of 2\% after $\sim 10^4$ communications compare to $\sim 5\times 10^2$ communications in the homogeneous case. Interestingly, we don't observe the same degradation in predictive performance as over-pruning occurs. 

The final performance of both PVI methods is worse than for the homogeneous split, achieving a test set error of 4\% and 6\% for synchronous and sequential PVI, respectively. These results reveal a shortcoming of sequential PVI, showing that it performs poorly in the presence of large numbers of inhomogeneous clients. The performance of synchronous PVI compares favourable with that of FedAVG, which achieves a test set error of $\sim 3\%$ after $10^3$ communication rounds \citep{mcmahan2017communication}. Considering that FedAVG produces a point estimate of the parameters, the results of synchronous PVI in the inhomogeneous setting are encouraging. 

Unsurprisingly, both BCM methods and VCL fail to learn an approximate posterior that performs better than random guessing.

\subsubsection{Time efficiency}
Figure \ref{fig:fmnist_homo_time} plots the predictive performance of federated learning methods, excluding global VI\footnote{Since global VI performs a single variational free-energy optimisation, it is by far the most time efficient. Yet, global VI is not a federated learning algorithm, so this comparison is unfair.}, as a function of elapsed time for the homogeneous split.

\begin{figure}[!h]
    \centering
    \includegraphics[width=\textwidth]{new/figs/fmnist/fmnist_homogeneous_pp_time.png}
    \caption[Predictive performance on the homogeneous split of the MNIST classification task as a function of time.]{Plots of the predictive performance of the federated learning schemes on the homogeneous split of the MNIST classification task as a function of time. The mean $\pm$ standard deviation computed using five random initialisations is shown. See text for details.}
    \label{fig:fmnist_homo_time}
\end{figure}

As expected, methods that are able to perform computation in parallel---synchronous PVI, asynchronous PVI and both BCM methods---are more time efficient than those that perform computation sequentially---sequential PVI, VCL and streaming VB. This is despite the use of damping for synchronous and asynchronous PVI, which means that a larger number of client updates are required for convergence of the approximate posterior.

Synchronous PVI and asynchronous PVI have the same initial rate of client updates, owing to the homogeneous distribution of dataset size amongst clients. As fewer gradients steps are performed for each local optimisation the rate of client updates increases for all PVI methods, with sequential, synchronous and asynchronous PVI converging to a rate of ?, ? and ? updates / second.

To highlight the benefits of asynchronous PVI over synchronous PVI, we consider another partition of the data in which the client-level distributions are homogeneous but have different $N_k$s. The performance plots are shown in Figure \ref{fig:fmnist_inhomo_size_time}.

\begin{figure}[!h]
    \centering
    \includegraphics[width=\textwidth]{new/figs/fmnist/fmnist_inhomogeneous_size_pp_time.png}
    \caption[Predictive performance on the inhomogeneous size split of the MNIST classification task.]{Plots of the predictive performance of the federated learning schemes on the inhomogeneous size split of the MNIST classification task. The split is constructed by randomly partitioning the 60,000 images into $K=5$ partitions of unequal size. The mean $\pm$ standard deviation computed using five random initialisations is shown.}
    \label{fig:fmnist_inhomo_size_time}
\end{figure}

Asynchronous PVI now has a far great initial rate of client updates than synchronous PVI. However, this is due to visiting the clients with the least amount of data far more frequently than the others. The learnt approximate posterior during this initial period approximates the true posterior conditioned on just a small fraction of the overall data, leading to poor predictive performance. Updates from the larger clients arrive at the same time for both asynchronous and synchronous PVI, at which point the predictive performance curves overlap. \textbf{This begs the question: should we ever use asynchronous PVI? Perhaps in the case of `faulty' communication channels, but not otherwise?} 

\subsection{More Plots}

\begin{itemize}
    \item Time efficiency plots for UCI datasets and mortality prediction.
    \item Effect of damping factor on PVI methods. 
    \item Plots illustrating which clients are updated and when for sequential, synchronous and asynchronous PVI. 
    \item Measure gradient of updated vs. time elapsed curves and include in text. Move figure to appendix and refer to it.
\end{itemize}

==> maths-preamble.tex <==
\RequirePackage{amsmath,amsthm,amssymb,amsbsy,algorithmic,mathtools,xcolor}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}


%Lowercase Bold Letters
\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfh}{\mathbf{h}}
\newcommand{\bfi}{\mathbf{i}}
\newcommand{\bfj}{\mathbf{j}}
\newcommand{\bfk}{\mathbf{k}}
\newcommand{\bfl}{\mathbf{l}}
\newcommand{\bfm}{\mathbf{m}}
\newcommand{\bfn}{\mathbf{n}}
\newcommand{\bfo}{\mathbf{o}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}

%Lowercase Bold Symbol Letters
\newcommand{\bsa}{\boldsymbol{a}}
\newcommand{\bsb}{\boldsymbol{b}}
\newcommand{\bsc}{\boldsymbol{c}}
\newcommand{\bsd}{\boldsymbol{d}}
\newcommand{\bse}{\boldsymbol{e}}
\newcommand{\bsf}{\boldsymbol{f}}
\newcommand{\bsg}{\boldsymbol{g}}
\newcommand{\bsh}{\boldsymbol{h}}
\newcommand{\bsi}{\boldsymbol{i}}
\newcommand{\bsj}{\boldsymbol{j}}
\newcommand{\bsk}{\boldsymbol{k}}
\newcommand{\bsl}{\boldsymbol{l}}
\newcommand{\bsm}{\boldsymbol{m}}
\newcommand{\bsn}{\boldsymbol{n}}
\newcommand{\bso}{\boldsymbol{o}}
\newcommand{\bsp}{\boldsymbol{p}}
\newcommand{\bsq}{\boldsymbol{q}}
\newcommand{\bsr}{\boldsymbol{r}}
\newcommand{\bss}{\boldsymbol{s}}
\newcommand{\bst}{\boldsymbol{t}}
\newcommand{\bsu}{\boldsymbol{u}}
\newcommand{\bsv}{\boldsymbol{v}}
\newcommand{\bsw}{\boldsymbol{w}}
\newcommand{\bsx}{\boldsymbol{x}}
\newcommand{\bsy}{\boldsymbol{y}}
\newcommand{\bsz}{\boldsymbol{z}}

%Lowercase Mathcal Letters
\newcommand{\mca}{\mathcal{a}}
\newcommand{\mcb}{\mathcal{b}}
\newcommand{\mcc}{\mathcal{c}}
\newcommand{\mcd}{\mathcal{d}}
\newcommand{\mce}{\mathcal{e}}
\newcommand{\mcf}{\mathcal{f}}
\newcommand{\mcg}{\mathcal{g}}
\newcommand{\mch}{\mathcal{h}}
\newcommand{\mci}{\mathcal{i}}
\newcommand{\mcj}{\mathcal{j}}
\newcommand{\mck}{\mathcal{k}}
\newcommand{\mcl}{\mathcal{l}}
\newcommand{\mcm}{\mathcal{m}}
\newcommand{\mcn}{\mathcal{n}}
\newcommand{\mco}{\mathcal{o}}
\newcommand{\mcp}{\mathcal{p}}
\newcommand{\mcq}{\mathcal{q}}
\newcommand{\mcr}{\mathcal{r}}
\newcommand{\mcs}{\mathcal{s}}
\newcommand{\mct}{\mathcal{t}}
\newcommand{\mcu}{\mathcal{u}}
\newcommand{\mcv}{\mathcal{v}}
\newcommand{\mcw}{\mathcal{w}}
\newcommand{\mcx}{\mathcal{x}}
\newcommand{\mcy}{\mathcal{y}}
\newcommand{\mcz}{\mathcal{z}}

%Uppercase Bold Letters
\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfC}{\mathbf{C}}
\newcommand{\bfD}{\mathbf{D}}
\newcommand{\bfE}{\mathbf{E}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\bfG}{\mathbf{G}}
\newcommand{\bfH}{\mathbf{H}}
\newcommand{\bfI}{\mathbf{I}}
\newcommand{\bfJ}{\mathbf{J}}
\newcommand{\bfK}{\mathbf{K}}
\newcommand{\bfL}{\mathbf{L}}
\newcommand{\bfM}{\mathbf{M}}
\newcommand{\bfN}{\mathbf{N}}
\newcommand{\bfO}{\mathbf{O}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfQ}{\mathbf{Q}}
\newcommand{\bfR}{\mathbf{R}}
\newcommand{\bfS}{\mathbf{S}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}

%Uppercase Mathcal Letters
\newcommand{\mcA}{\mathcal{A}}
\newcommand{\mcB}{\mathcal{B}}
\newcommand{\mcC}{\mathcal{C}}
\newcommand{\mcD}{\mathcal{D}}
\newcommand{\mcE}{\mathcal{E}}
\newcommand{\mcF}{\mathcal{F}}
\newcommand{\mcG}{\mathcal{G}}
\newcommand{\mcH}{\mathcal{H}}
\newcommand{\mcI}{\mathcal{I}}
\newcommand{\mcJ}{\mathcal{J}}
\newcommand{\mcK}{\mathcal{K}}
\newcommand{\mcL}{\mathcal{L}}
\newcommand{\mcM}{\mathcal{M}}
\newcommand{\mcN}{\mathcal{N}}
\newcommand{\mcO}{\mathcal{O}}
\newcommand{\mcP}{\mathcal{P}}
\newcommand{\mcQ}{\mathcal{Q}}
\newcommand{\mcR}{\mathcal{R}}
\newcommand{\mcS}{\mathcal{S}}
\newcommand{\mcT}{\mathcal{T}}
\newcommand{\mcU}{\mathcal{U}}
\newcommand{\mcV}{\mathcal{V}}
\newcommand{\mcW}{\mathcal{W}}
\newcommand{\mcX}{\mathcal{X}}
\newcommand{\mcY}{\mathcal{Y}}
\newcommand{\mcZ}{\mathcal{Z}}




%Common domains, S,R,C,Z,N...
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}



%Theorem Environments

\newtheorem{prop}{Proposition}[section]
% \newtheorem{miniprop}{Mini-Proposition}
% \newtheorem{thm}{Theorem}
\newtheorem{property}{Property}[section]

% \newtheorem{cor}{Corollary}
% \newtheorem{lem}{Lemma}

% \newtheorem{ex}{Example}
% \newtheorem{rem}{Remark}
% \newtheorem{observation}{Observation}
% \newtheorem{defi}{Definition}

% \Crefname{thm}{Theorem}{Theorems}
% \Crefname{lem}{Lemma}{Lemmas}
% \Crefname{prop}{Proposition}{Propositions}


%Commonly used matrices for GPs/Sparse Inference
\newcommand{\Kff}{\bfK_{\bf ff}}
\newcommand{\tilk}{\tilde{\bfK}_{\bf ff}}
\newcommand{\Qff}{\bfQ_{\bf ff}}
\newcommand{\KZ}{\bfK_{\bf Z}}
\newcommand{\Kuf}{\bfK_{\bf uf}}
\newcommand{\Kuu}{\bfK_{\bf uu}}



%miscellaneous
\def\*#1{\boldsymbol{\mathbf{#1}}}

\newcommand{\bfPsi}{\boldsymbol{\Psi}}
\newcommand{\bfpsi}{\boldsymbol{\psi}}
\newcommand{\Ahat}{\mathbf{\hat{A}}}
\newcommand{\Ghat}{\mathbf{\hat{G}}}
\newcommand{\Khat}{\mathbf{\hat{K}}}
\newcommand{\bfYp}{\mathbf{Y_{\bullet}}}
\newcommand{\bfGamma}{\boldsymbol{\Gamma}}
\newcommand{\ddx}{\frac{d}{dx}}

\newcommand{\sn}{\sigma_{n}}

\newcommand{\mcLl}{\mathcal{L}_\text{lower}}
\newcommand{\mcLu}{\mathcal{L}_\text{upper}}
\newcommand{\dxdt}{\frac{\partial{x}}{\partial{t}}}
\newcommand{\dt}{\partial{t}}
\newcommand{\ddt}{\frac{\partial}{\partial{t}}}
\newcommand{\ddxd}{\frac{\partial}{\partial{x_d}}}
\newcommand{\ddxdp}{\frac{\partial}{\partial{x_{d'}}}}

\newcommand{\FT}{\frac{1}{\sqrt{2\pi}}\int g(x) e^{-i\omega x}dx}

\newcommand{\sgn}{\text{sgn}}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\eqdef}{=\vcentcolon}

\newcommand{\transpose}{^\mathrm{\textsf{\tiny T}}}
\newcommand{\ExpSymb}{\mathbb{E}}
\newcommand{\Exp}[2]{\ExpSymb_{#1}\left[#2\right]}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\GP}{\mathcal{GP}}
\newcommand{\FromDist}{\sim}
\newcommand{\KL}[2]{\mathrm{KL}\left( {#1}\ \|\ {#2} \right)}
\newcommand{\KLint}[3]{\int #1 \log \left( \frac{#1}{#2} \right) \calcd{#3}}
\newcommand{\Normal}[3]{\mcN\left( {#1} ; {#2}, {#3}\right)}
\newcommand{\entropy}[1]{\mathcal{H}\left( #1 \right)}
\newcommand{\given}{\,\vert \,}
\newcommand{\quadform}[2]{{#2}\transpose{#1}{#2}}
\newcommand{\deriv}[2]{\frac{d {#1}}{d {#2}}}
\newcommand{\derivsquared}[2]{\frac{d^2 {#1}}{d {#2}^2}}
\newcommand{\derivsquaredvec}[2]{\frac{d^2 {#1}}{d {#2} d{#2}^T}}
\newcommand{\normaldist}[3]{\mcN\left(#1; #2, #3\right)}

\newcommand{\cov}{\text{cov}}

==> preamble.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{multirow}       % multirow...
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{natbib}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage[inline]{enumitem}       % nice lists.
\usepackage{parskip}        % skip paragraphs.
\PassOptionsToPackage{round}{natbib}
\usepackage{pdflscape}         % allows for landscape
\let\proof\relax
\let\endproof\relax
\RequirePackage{amsmath,amsfonts,amssymb,amsthm}
\usepackage{afterpage}
\usepackage{algorithm,algorithmic}
\usepackage[usenames, dvipsnames]{color}
\usepackage{mathtools}

\usepackage{cancel}
\usepackage{caption}
\usepackage{rotating}
\usepackage{lipsum}

\usepackage{subcaption}
\usepackage{cleveref}

\def\therefore{\boldsymbol{\text{ }
\leavevmode
\lower0.4ex\hbox{$\cdot$}
\kern-.5em\raise0.7ex\hbox{$\cdot$}
\kern-0.55em\lower0.4ex\hbox{$\cdot$}
\thinspace\text{ }}}

%
\usepackage{xargs}                      % Use more than one optional parameter in a new commands
\usepackage[pdftex,dvipsnames]{xcolor}  % Coloured text etc.
\usepackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}
\newcommandx{\unsure}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommandx{\change}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommandx{\info}[2][1=]{\todo[linecolor=OliveGreen,backgroundcolor=OliveGreen!25,bordercolor=OliveGreen,#1]{#2}}
\newcommandx{\improvement}[2][1=]{\todo[linecolor=Plum,backgroundcolor=Plum!25,bordercolor=Plum,#1]{#2}}
\newcommandx{\thiswillnotshow}[2][1=]{\todo[disable,#1]{#2}}
%

% make plus and minus symbol
\makeatletter
\newcommand{\mypm}{\mathbin{\mathpalette\@mypm\relax}}
\newcommand{\@mypm}[2]{\ooalign{%
  \raisebox{.1\height}{$#1+$}\cr
  \smash{\raisebox{-.6\height}{$#1-$}}\cr}}
\makeatother

% for enumitem
\usepackage{tikz}
\newcommand*\whitecirc[1]{%
\begin{tikzpicture}[baseline=(C.base)]
\node[draw,circle,inner sep=-1pt,minimum size=3ex](C) {#1};
\end{tikzpicture}}

\newcommand*\blackcirc[1]{%
\begin{tikzpicture}[baseline=(C.base)]
\node[draw,circle,inner sep=-1pt,minimum size=3ex,fill=black,text=white](C) {#1};
\end{tikzpicture}}

% \newcommand\blackcirc[1]{%
%   \tikz[baseline=(X.base)] 
%     \node (X) [draw, shape=circle, inner sep=-1pt, fill=black, text=white] {\strut #1};%
% }
